Quasiparticle Generation-Recombination Noise in the Limit of Low Detector Volume

We have measured the quasiparticle generation-recombination (GR) noise in aluminium lumped element kinetic inductors with a wide range of detector volumes at various temperatures. The basic detector consists of meandering inductor and interdigitated capacitor fingers. The inductor volume is varied from 2 to 153 {\mu}m^{3} by changing the inductor width and length to maintain a constant inductance. We started with measuring the power spectrum density (PSD) of the detectors frequency noise which is a function of GR noise and we clearly observed the spectrum roll off at 10 kHz which corresponds to the quasiparticle lifetime. Using data from a temperature sweep of the resonator frequency we convert the frequency fluctuation to quasiparticle fluctuation and observe its strong dependence on detector volume: detectors with smaller volume display less quasiparticle noise amplitude. Meanwhile we observe a saturated quasiparticle density at low temperature from all detectors as the quasiparticle life time {\tau}qp approaches a constant value at low temperature.

==> authors.tex <==
\author{
J.~Li\textsuperscript{1},
P.~S.~Barry\textsuperscript{2, 1},
T.~Cecil\textsuperscript{1},
C.~L.~Chang\textsuperscript{1, 3, 4},
K.~Dibert\textsuperscript{3},
R.~Gualtieri\textsuperscript{1},
J.~Zhang\textsuperscript{1},
M.~Lisovenko\textsuperscript{1},
Z.~Pan\textsuperscript{1},
V.~Yefremenko\textsuperscript{1}
G.~Wang\textsuperscript{1},
and ~J.~Zhang\textsuperscript{1},
% Affiliations

\institute{
\textsuperscript{1}{Argonne National Laboratory, 9700 South Cass Avenue., Argonne, IL, 60439, USA} \\
\textsuperscript{2}{School of Physics and Astronomy, Cardiff University, Cardiff CF24 3YB, UK} \\
\textsuperscript{3}{Dept. of Astronomy \& Astrophysics, U. Chicago, 5640 South Ellis Avenue, Chicago, IL, 60637, USA} \\
\textsuperscript{4}{Kavli Institute for Cosmological Physics, U. Chicago, 5640 South Ellis Avenue, Chicago, IL, 60637, USA} \\
}

}

==> authors0.tex <==
\author{
J.~Li\textsuperscript{1},
P.~S.~Barry\textsuperscript{1},
T. Cecil\textsuperscript{1},
C.~L.~Chang\textsuperscript{1,2,3},
K. Dibert\textsuperscript{2},
R. Gualtieri\textsuperscript{1},
M. Lisovenko,\textsuperscript{1},
Z.~Pan\textsuperscript{1},
V.~Yefremenko\textsuperscript{1},
G. Wang\textsuperscript{1},
J. Zhang\textsuperscript{1},

\institute{
\textsuperscript{1}{Argonne National Laboratory, 9700 South Cass Avenue., Argonne, IL, 60439, USA} \\
\textsuperscript{2}{Dept. of Astronomy \& Astrophysics, U. Chicago, 5640 South Ellis Avenue, Chicago, IL, 60637, USA} \\
\textsuperscript{3}{Kavli Institute for Cosmological Physics, U. Chicago, 5640 South Ellis Avenue, Chicago, IL, 60637, USA} \\
}
}
